Guidance Through Surrogate: Towards a Generic Diagnostic Attack

Adversarial training is an effective approach to make deep neural networks robust against adversarial attacks. Recently, different adversarial training defenses are proposed that not only maintain a high clean accuracy but also show significant robustness against popular and well studied adversarial attacks such as PGD. High adversarial robustness can also arise if an attack fails to find adversarial gradient directions, a phenomenon known as `gradient masking'. In this work, we analyse the effect of label smoothing on adversarial training as one of the potential causes of gradient masking. We then develop a guided mechanism to avoid local minima during attack optimization, leading to a novel attack dubbed Guided Projected Gradient Attack (G-PGA). Our attack approach is based on a `match and deceive' loss that finds optimal adversarial directions through guidance from a surrogate model. Our modified attack does not require random restarts, large number of attack iterations or search for an optimal step-size. Furthermore, our proposed G-PGA is generic, thus it can be combined with an ensemble attack strategy as we demonstrate for the case of Auto-Attack, leading to efficiency and convergence speed improvements. More than an effective attack, G-PGA can be used as a diagnostic tool to reveal elusive robustness due to gradient masking in adversarial defenses.

==> tables/computational_cost_analysis.tex <==
\begin{table}[!t]
	\centering%\small
		\setlength{\tabcolsep}{7pt}
		\scalebox{1}[1]{
		\begin{tabular} { ccccc }
			\toprule
			\rowcolor{Gray}
			& &\multicolumn{3}{c}{ResNet50} \\
			\rowcolor{Gray} 
			\multirow{-2}{*}{Dataset}&\multirow{-2}{*}{Attack} & $\epsilon=2.0$& $\epsilon=4.0$& $\epsilon=8.0$\\
			 \hline
			 \multirow{3}{*}{ImageNet-5k} &PGD  & 67.6 & 50.7  &32.1\\
			 & Auto-Attack  & 65.6 & 47.5&\textbf{30.0}\\
		  & G-PGA & \textbf{64.1} & \textbf{47.3}  &\textbf{30.0}\\
			 \bottomrule
	\end{tabular}}
	\caption{ \emph{Effectiveness of G-PGA on ImageNet:} We evaluate adversarially trained ResNet50 models from \cite{salman2020adversarially} against different attacks including G-PGA (ours). Note that evaluation perturbation budget for each model is the same as its training perturbation budget % on which the model was trained 
	\eg ResNet50 trained on $\epsilon=2.0$ is evaluated with the perturbation budget of $\epsilon=2.0$. The surrogate model used in G-PGA is a naturally trained ResNet50. G-PGA performs favorably in comparison to Auto-Attack while being computationally efficient (Table \ref{tab:computational_comparison_with_AA_rebuttal}).  }
	\label{tab: imagenet_results}
\end{table}


\begin{table}[!t]
	\centering\small
		\scalebox{0.85}{
		\begin{tabular}{lcccc}
				\toprule
					\rowcolor{Gray}
			Attack & CIFAR10 & CIFAR100 & SVHN & ImageNet-5k\\
			\midrule
            Auto-Attack & 682.5&2598.2&1774.5&12.8$\times$10$^3$\\
            Auto-Attack (Cheap) & 148.5&581.0&388.7&4252 \\ 
            Proposed Attack &\textbf{ 87.0} & \textbf{88.2}&\textbf{226.2}&\textbf{240}\\
			\bottomrule
	\end{tabular}}
	\caption{Computational time (minutes, lower is better) is noted on a Tesla-V100. Attacks ran on $l_\infty$ adversarially trained models at $\epsilon=8$. WideResNet is used for CIFAR10, CIFAR100, and SVHN datasets while ResNet50 is used for ImageNet-5k. Results are reported using the test samples for each dataset with a batch size of 100.}
	\label{tab:computational_comparison_with_AA_rebuttal}
\end{table}

